Corex: Pushing the Boundaries of Complex Reasoning through Multi-Model Collaboration

Large Language Models (LLMs) are evolving at an unprecedented pace and have exhibited considerable capability in the realm of natural language processing (NLP) with world knowledge. Benefiting from ultra-large-scale training corpora, a single LLM can manage typical NLP tasks competently. However, its performance in executing reasoning tasks is still confined by the limitations of its internal representations. To push this boundary further, we introduce Corex in this paper, a suite of novel general-purpose strategies that transform LLMs into autonomous agents pioneering multi-model collaborations for complex task-solving. Inspired by human behaviors, Corex is constituted by diverse collaboration paradigms including Debate, Review, and Retrieve modes, which collectively work towards enhancing the factuality, faithfulness, and reliability of the reasoning process. These paradigms foster task-agnostic approaches that enable LLMs to ''think outside the box,'' thereby overcoming hallucinations and providing better solutions. Through extensive experiments across four different types of reasoning tasks, we demonstrate that orchestrating multiple LLMs to work in concert yields substantially better performance compared to existing methods. Further results and in-depth analysis demonstrate the cost-effectiveness of our method, facilitating collaboration among different LLMs and promoting annotation efficiency.

==> appendices/eval-details.tex <==
\section{Evaluation Details}
\label{appendix:eval-details}


prompts

==> sections/results/method-comparison.tex <==
% \begin{table}[!ht]
%     \centering
%     \caption{ A comparison of \ours to other recent prompting strategies.}
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{lccccc}
%         \toprule
%         \textbf{Feature} & \makecell{\textbf{\ours} \\ (our work)} & \makecell{ \textbf{PAL} \\\citep{gao2022pal} } & 
%         \makecell{ \textbf{Progressive-Hint Prompting} \\ \citep{zheng2023php} } & \makecell{ \textbf{Chain-of-Knowledge} \\\citep{wang2023cok} } & \makecell{ \textbf{Tree-of-Thoughts}\\\citep{yao2023tree} } 
%         \\
%          \cmidrule(lr){1-1}  \cmidrule(lr){2-2}  \cmidrule(lr){3-3}  \cmidrule(lr){4-4}  \cmidrule(lr){5-5} \cmidrule(lr){6-6}
%           Task Agnostic?    & \greencheck & \redcross   & \redcross    & \greencheck & \greencheck  \\ 
%           Multiple Chains?  & \greencheck & \redcross   & \redcross    & \redcross   & \greencheck  \\ 
%           Delegation?       & \greencheck & \greencheck & \redcross    & \redcross   & \redcross  \\ 
%           Reference Free?   & \greencheck & \greencheck & \greencheck  & \redcross   & \greencheck  \\ 
%          \bottomrule
%     \end{tabular}
%     }
%     \label{tab:dataset_comparison}
% \end{table}


\begin{table}[!ht]
    \centering
    \caption{A comparison of \ours to other recent prompting strategies.}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lccccc}
        \toprule
        \textbf{Feature} & \makecell{\textbf{\ours} \\ (our work)} & \makecell{ \textbf{MAD} \\\citep{liang2023encouraging} } & 
        \makecell{ \textbf{PHP} \\ \citep{zheng2023php} } & \makecell{ \textbf{CoK} \\\citep{wang2023cok} } & \makecell{ \textbf{ToT}\\\citep{yao2023tree} } 
        \\
         \cmidrule(lr){1-1}  \cmidrule(lr){2-2}  \cmidrule(lr){3-3}  \cmidrule(lr){4-4}  \cmidrule(lr){5-5} \cmidrule(lr){6-6}
          Task Agnostic?    & \greencheck & \redcross   & \redcross    & \greencheck & \greencheck  \\ 
          Multiple Chains?  & \greencheck & \redcross   & \redcross    & \redcross   & \greencheck  \\ 
          Multiple LLMs?    & \greencheck & \greencheck   & \redcross    & \redcross   & \redcross  \\ 
          Task Delegation?  & \greencheck & \redcross & \redcross    & \redcross   & \redcross  \\ 
          Reference Free?   & \greencheck & \greencheck & \greencheck  & \redcross   & \greencheck  \\ 
         \bottomrule
    \end{tabular}
    }
    \label{tab:maethod_comp}
    \vspace{-1em}
\end{table}

==> sections/results/overall.tex <==
\begin{table}[ht]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lllllll}
\toprule
           & Mathematical Reasoning & Question Answering  & Table Understanding  & Big-Bench & Avg.     \\ 
\midrule
CoT       & -  & - & - & - & -  \\
CoT-SC(10)       & -  & - & - & - & -  \\
ComplexCoT(5)   & -  & - & - & - & -  \\
% PAL             & -  & - & - & - & -  \\
\midrule 
\crd            & -  & - & - & - & -   \\  
\crnl           & -  & - & - & - & -   \\  
\crcode         & -  & - & - & - & -   \\   
\crrt           & -  & - & - & - & -   \\  
\bottomrule
\end{tabular}
}
\caption{Comparison of accuracy on seven math reasoning datasets using various \crraw modes and \sqs{TBD} strong baselines. The best results are indicated in bold. \sqs{no AuQA} \sqs{Details/breakdown are in Table2 3 4 5 respectively}}
\label{tab:overall-result}
\end{table}


 




==> sections/results/table-results.tex <==
% \begin{wraptable}[26]{r}{0.495\textwidth}
% \vspace{-0.75em}
% \centering
% \caption{Comparison of performance on FinQA and ConvFinQA between \crraw and strong baselines.}
% % \setlength{\tabcolsep}{1pt}
% \resizebox{0.95\linewidth}{!}{
% \begin{tabular}{lccc}
% \toprule
%                 & FinQA & ConvFinQA  & Avg.     \\ 
% \midrule
% CoT             & 46.1  & 50.4 & 48.3  \\
% CoT-SC(10)      & 52.7  & \underline{57.2} & 54.9  \\
% PAL             & 54.3  & 50.8 & 52.9   \\
% \midrule 
% \crd            & 50.2                    & 56.7             & 53.5   \\  
% \crnl           & 52.5                    & 52.3             & 52.4   \\  
% \crcode         & \textbf{55.9}           & 54.2             & \underline{55.1}   \\   
% \crrt           & \underline{55.4}        & \textbf{57.7}    & \textbf{56.6}   \\  
% \bottomrule
% \end{tabular}
% }
% \label{tab:table-result}
% \vspace{-1em}
% \end{wraptable}


% \begin{wrapfigure}[26]{r}{0.42\textwidth}
% \vspace{-5mm}
% \includegraphics[width=0.42\textwidth]{figures/retrieve-illustration.pdf}
% \vspace{-6mm}
% \caption{Illustration of reviewing erroneous code generated by other agents (first round).}
% \label{fig:retrieve-illustration}
% \end{wrapfigure}


% finqa pal 0.54925

% \paragraph{Commonsense \& Factual Reasoning.}
% \begin{wraptable}{rht}{0.55\textwidth}
% % \begin{table}[t]
% \centering
% \setlength{\tabcolsep}{1pt}
% \caption{Accuracy on arithmetic reasoning tasks. 
% }
% \label{tab:main_results_2}
% \resizebox{\linewidth}{!}{
% % \begin{small}
% \begin{tabular}
% % {lccccccccc}
% {p{0.20\textwidth}p{0.12\textwidth}p{0.12\textwidth}p{0.1\textwidth}p{0.12\textwidth}}
% \toprule
% Model & GSM8K   & SVAMP & AQuA & MultiArith  \\
% \midrule
% Fine-tuning  &  55.0 & 57.4  & 37.9 & - \\
% \midrule
% Zero-Shot SP  & 10.4 & 58.8  & 22.4 &  17.7  \\
% Zero-Shot CoT  & 40.7  & 62.1 & 33.5 & 78.7  \\
% Few-Shot SP & 15.6 & 65.7 & 24.8 & 33.8  \\
% Manual CoT   & 46.9 & 68.9 & 35.8 & 91.7  \\
% Auto-CoT & 47.9  & 69.5  & 36.5   & 92.0 \\
% \midrule
% CoK &  \textbf{48.9}  &  \textbf{69.9}  &  \textbf{37.8}  & \textbf{94.6} \\
% \bottomrule
% \end{tabular}
% % \end{small}
% }
% % \vspace{-4mm}
% \end{wraptable}
 
% \begin{wraptable}{r}{0.4\textwidth}
% % \vspace{-3.6mm}
%     \centering
%         \caption{Accuracy (\%) of different sampling methods. Symbol $\dagger$  indicates using training sets with annotated reasoning chains. \label{tab:preliminary}}
%     % \vspace{-2mm}
%     \setlength{\tabcolsep}{2pt}
% \begin{tabular}{l|c|cc}\toprule
%  {Method} & {MultiArith} & {GSM8K} & {AQuA}  \\\midrule
%  Zero-Shot-CoT & 78.7 & 40.7 & 33.5  \\
%  Manual-CoT & \textbf{91.7} & 46.9 & 35.8$\dagger$ \\
% \midrule
% Random-Q-CoT & 86.2 & 47.6$\dagger$ & 36.2$\dagger$ \\
% Retrieval-Q-CoT & 82.8 & \textbf{48.0}$\dagger$ & \textbf{39.7}$\dagger$ \\
% \bottomrule
% \end{tabular}
% % \vspace{-2mm}
% \end{wraptable}
